PinLanding: Content-First Keyword Landing Page Generation via Multi-Modal AI for Web-Scale Discovery

Online platforms like Pinterest hosting vast content collections traditionally rely on manual curation or user-generated search logs to create keyword landing pages (KLPs) -- topic-centered collection pages that serve as entry points for content discovery. While manual curation ensures quality, it doesn't scale to millions of collections, and search log approaches result in limited topic coverage and imprecise content matching. In this paper, we present PinLanding, a novel content-first architecture that transforms the way platforms create topical collections. Instead of deriving topics from user behavior, our system employs a multi-stage pipeline combining vision-language model (VLM) for attribute extraction, large language model (LLM) for topic generation, and a CLIP-based dual-encoder architecture for precise content matching. Our model achieves 99.7% Recall@10 on Fashion200K benchmark, demonstrating strong attribute understanding capabilities. In production deployment for search engine optimization with 4.2 million shopping landing pages, the system achieves a 4X increase in topic coverage and 14.29% improvement in collection attribute precision over the traditional search log-based approach via human evaluation. The architecture can be generalized beyond search traffic to power various user experiences, including content discovery and recommendations, providing a scalable solution to transform unstructured content into curated topical collections across any content domain.

==> Sections/technical_implementation.tex <==
\subsection{Technical Implementation \textcolor{blue}{TODO: delete, merge into the previous section}}

\subsubsection{Vision LLM for Attribute Generation}

We use GPT-4-V as the vision LLM for attribute generation. Product images, along with associated text information such as title, description, price, and user-provided tags, are passed to GPT-4-V's API. 

\paragraph{Prompt Engineering}
In the prompt, we instruct GPT to output a comprehensive set of attributes for each specific category, including product type, color, style, material, usage occasion, season, and more, in a structured JSON format. We found that by asking GPT to generate attributes for each category, rather than allowing it to output attributes freely, it is more likely to provide detailed and well-organized information.

\subsubsection{CLIP for Content Matching}

CLIP\cite{clip} is a vision-language model pre-trained to associate images with text using contrastive learning. It maximizes similarity between matching image-text pairs and minimizes it for non-matching pairs.

\paragraph{Model Adaptation}
Although our content matching task is similar to CLIP's pretraining image-text matching, it differs due to the multimodal nature of the inputs—specifically, matching a product (image + text) with an attribute (text). This requires adapting the CLIP architecture. As shown in Figure \ref{fig:clip}, product images and descriptions are encoded with an image encoder and a text encoder, respectively, while attributes are encoded with a separate text encoder. All encoders are based on Vision Transformers and Text Transformers, using CLIP's pretraining weights. The product image and text embeddings are combined into a single product embedding. Using CLIP's contrastive loss, matching product-attribute pairs are encouraged to have higher similarity between their embeddings, while non-matching pairs are pushed to have lower similarity. This allows the adapted CLIP model to learn the relationships between products and attributes.
During inference, for each new product, we calculate its similarity with each attribute and apply a threshold. Attributes with similarities above the threshold are considered relevant to the product.

\paragraph{Post-Processing Weight}
Here we observed an issue with CLIP's predictions. In training data, there is a natural long tail in product-attribute relationships–some attributes, like "color: white," match many products, while others, like "details: embroidered hem," match only a few. While this is reasonable, CLIP's predictions tend to smooth this long tail, downplaying common attributes and overstating rare ones. To correct this, we apply a simple post-processing weight to attributes based on their popularity in the training data, ensuring the predictions align more closely with the training distribution.



\subsubsection{LLM for Query Generation}

We use GPT-4 as the LLM to connect discrete attributes into a coherent, natural-sounding query for the KLP title, while also evaluating the query's searchability to provide scores for quality filtering.

\paragraph{Prompt Engineering}

We provide multiple examples in the prompt to guide the LLM in performing three tasks:

\begin{enumerate}
    \item \textit{Validate the attribute list}. The LLM checks for redundancy or irrelevant keywords. For instance, an attribute list such as ``l2 category: rings, style: elegant, shape: round" is considered invalid since rings are typically round, thus preventing the generation of unnatural queries.
    \item \textit{Generate a concise, natural-sounding search query}. The LLM generates queries based on the attributes, such as ``Michael Kors Black Sunglasses" or ``Black Long Sleeve Dress for New Year's Eve."
    \item \textit{Rate the searchability}. The LLM rates the generated query on a scale from 1 to 5. Queries that are overly specific, such as ``Trail Running Shoes with Branded Insole and White Sole," are assigned lower scores due to their rarity in user searches.
\end{enumerate}


\paragraph{Quality Filtering}

After obtaining the LLM output, we filter out attribute lists marked as invalid and queries with low searchability scores. We keep only the high-quality queries generated from valid attribute lists, and use them as titles for new KLPs. The products associated with the corresponding attribute lists serve as the product feed for these KLPs.

% \paragraph{Coverage optimization}


